Sycophancy Mitigation Through Reinforcement Learning with Uncertainty-Aware Adaptive Reasoning Trajectories

Despite the remarkable capabilities of large language models, current training paradigms inadvertently foster \textit{sycophancy}, i.e., the tendency of a model to agree with or reinforce user-provided information even when it's factually incorrect. To address this challenge, we introduce \textbf{SMART} (Sycophancy Mitigation through Adaptive Reasoning Trajectories), which reframes sycophancy as a \textit{reasoning optimization problem} rather than an output alignment issue. SMART is a two-stage framework comprising: (1) Uncertainty-Aware Adaptive Monte Carlo Tree Search (UA-MCTS), which dynamically adjusts model exploration based on state-level uncertainty to collect high-quality, diverse reasoning trajectories alongside both stepwise progress and final outcome rewards; and (2) progress-based reinforcement learning, which fine-tunes the model using the collected trajectories and reward signals to reinforce effective reasoning patterns. Through extensive experiments, we show that SMART significantly reduces sycophantic behavior while preserving strong performance on out-of-distribution inputs and maintaining general capabilities. These results underscore the importance of optimizing internal reasoning mechanisms to build more truthful and aligned AI assistants.

==> latex/Figures/method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{latex/Figures/fig1.pdf}
    \caption{ \textbf{SMART Framework Overview}. \textbf{(a)~Generation of Reasoning Trajectories:} UA-MCTS dynamically explores reasoning paths from initial states using uncertainty-aware adaptive exploration. Progress rewards ($r_{prog}$) are assigned at each reasoning step based on information gain, while outcome rewards ($r_{out}$) evaluate final answers. \textbf{(b)~Reasoning-Guided RL:} The policy model is then trained using both progress and outcome rewards collected from UA-MCTS trajectories, optimizing reasoning processes rather than just final outputs to mitigate sycophantic behavior.}
    \label{fig:method}
\end{figure*}
